The River Method

We introduce River, a novel Condorcet-consistent voting method that is based on pairwise majority margins and can be seen as a simplified variation of Tideman's Ranked Pairs method. River is simple to explain, simple to compute even 'by hand', and gives rise to an easy-to-interpret certificate in the form of a directed tree. Like Ranked Pairs and Schulze's Beat Path method, River is a refinement of the Split Cycle method and shares with those many desirable properties, including independence of clones. Unlike the other three methods, River satisfies a strong form of resistance to agenda-manipulation that is known as independence of Pareto-dominated alternatives.

==> property_table_axioms.tex <==
\definecolor{MexicanRed}{rgb}{0.682,0.141,0.176}%{1,1,1}%{0,0,0}    %dark line  rgb(173,38,44)
\definecolor{Punch}{rgb}{1,1,1}%{0.878,0.274,0.294}         %light line rgb(201,111,116)
\definecolor{MyPink}{RGB}{231,180,181}        %dark row   rgb(231,180,181)
\definecolor{Shilo}{RGB}{244,213,215}          %light row  
\definecolor{White}{rgb}{1,1,1}
%------------------------------------------------------------------------------------------------
\definecolor{MyPinkDark}{RGB}{221, 149, 150}        % DARKER dark row   rgb()
\definecolor{MyPinkLight}{RGB}{238, 202, 203}        % LIGHTER dark row   
\definecolor{ShiloDark}{RGB}{235, 177, 180}          % DARKER light row
\definecolor{ShiloLight}{RGB}{247, 226, 227}          % LIGHTER light row  
\definecolor{Grayy}{RGB}{242, 242, 242}
%------------------------------------------------------------------------------------------------
\definecolor{DarkLine}{RGB}{156,156,156}    %dark line  
\definecolor{LightLine}{rgb}{1,1,1}         %light line 
\definecolor{DarkRow}{RGB}{222, 222, 222}   %dark row 
\definecolor{LightRow}{RGB}{242, 242, 242}  %light row  
\definecolor{White}{rgb}{1,1,1}
%------------------------------------------------------------------------------------------------
\definecolor{DarkRowRiver}{RGB}{212,212,212}        % DARKER dark row   rgb()
\definecolor{LightRowRiver}{RGB}{232,232,232}          % DARKER light row
\definecolor{Grayy}{RGB}{242, 242, 242}
\newcommand{\svipda}{(\y*)}
\newcommand{\RM}{RV}
%------------------------------------------------------------------------------------------------
%\crefname{prop:osition}{Prop.}{Prop.}
\begin{table}[t]
\centering
\begin{tblr}{
  width = \linewidth,
  colspec = {@{}Q[152]Q[37]Q[37]Q[37]Q[37]Q[37]},
  row{even} = {DarkRow},
  row{odd} = {LightRow},
  row{1} = {White},
  column{1}= {White},
  column{even} = {c},
  column{odd} = {c},
  column{1} = {l},
  vline{1-7} = {-}{LightLine},
  hline{1-20} = {-}{LightLine},
  hline{2,6,10} = {-}{DarkLine},
  hline{1,13} = {-}{0.1em,DarkLine},
}
    & \SC &  \SV & \RP & \BP & \SetCell{bg=Grayy}\RM \\
%\hyperref[def:AnonymityandNeutrality]{Anonymity}
Anonymity
    & \y  &  \hphantom{*}\y*   & \hphantom{*}\y* & \y & \SetCell{bg=DarkRowRiver} \hphantom{*}\y*\\
%\hyperref[def:AnonymityandNeutrality]{Neutrality}
Neutrality
    & \y  &  \hphantom{*}\y*   & \hphantom{*}\y* & \y & \SetCell{bg=LightRowRiver}\hphantom{*}\y*\\
% Reversal Symm.
%     & \y & \y & \y & \y & \SetCell{bg=DarkRowRiver}\y \\
Monotonicity
    & \y & \n & \y & \y & \SetCell{bg=LightRowRiver}\y \\
Condorcet Winner
    & \y & \y & \y & \y & \SetCell{bg=DarkRowRiver}\y \\
Condorcet Loser
    & \y & \y & \y & \y & \SetCell{bg=LightRowRiver}\y \\
Smith criterion
    & \y & \y & \y & \y & \SetCell{bg=DarkRowRiver}\y \\
Pareto efficiency
    & \y & \y & \y & \y & \SetCell{bg=LightRowRiver}\y \\
ISDA 
    & \y  & $\hphantom{\circ}\y^\circ$ & \y & \y & \SetCell{bg=DarkRowRiver}\hphantom{*}\y \\
IPDA
    & \n  & \n & \n & \n & \SetCell{bg=LightRowRiver}\hphantom{*}\y*
\end{tblr}
\caption{Overview of the properties for Split Cycle and refinements.
``\y'' indicates the property is satisfied for general profiles.
``\y*'' indicates the property is satisfied for general profiles with a suitable tie-breaker.
``$\y^\circ$'' indicates the property is satisfied for uniquely weighted profiles.
``\n'' indicates the property is violated even for uniquely weighted profiles.
For all results not concerning River or IPDA, %, i.e., everything but the last column and last row, 
we refer to \cite{holliday2020split}.}
\label{tab:BasicAxioms}
\end{table}
